Divert More Attention to Vision-Language Tracking

Relying on Transformer for complex visual feature learning, object tracking has witnessed the new standard for state-of-the-arts (SOTAs). However, this advancement accompanies by larger training data and longer training period, making tracking increasingly expensive. In this paper, we demonstrate that the Transformer-reliance is not necessary and the pure ConvNets are still competitive and even better yet more economical and friendly in achieving SOTA tracking. Our solution is to unleash the power of multimodal vision-language (VL) tracking, simply using ConvNets. The essence lies in learning novel unified-adaptive VL representations with our modality mixer (ModaMixer) and asymmetrical ConvNet search. We show that our unified-adaptive VL representation, learned purely with the ConvNets, is a simple yet strong alternative to Transformer visual features, by unbelievably improving a CNN-based Siamese tracker by 14.5% in SUC on challenging LaSOT (50.7% > 65.2%), even outperforming several Transformer-based SOTA trackers. Besides empirical results, we theoretically analyze our approach to evidence its effectiveness. By revealing the potential of VL representation, we expect the community to divert more attention to VL tracking and hope to open more possibilities for future tracking beyond Transformer. Code and models will be released at https://github.com/JudasDie/SOTS.

==> tables/got10k.tex <==
\begin{table}[!t]
	\centering
	\vspace{-3mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\opt}[1]{\textbf{\textcolor{violet}{#1}}}
	\newcommand{\fast}[1]{\textbf{\textcolor{orange}{#1}}}
	\newcommand{\dist}{\hspace{3pt}}%
	\renewcommand\arraystretch{1.2}
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        % 	\toprule
        	\hline
        	           &    &STARK &Tr   &     &Auto   & Siam & Pr  &  &  &\textit{\textbf{Siam}}  &  &SNLT  &Siam &Siam\\
        	           & \textbf{VLT}$_{\mathrm{TT}}$     &st50 &DiMP    & \textit{\textbf{TransT}} &Match & R-CNN & DiMP & \textbf{VLT}$_{\mathrm{SCAR}}$ & Ocean   &\textit{\textbf{CAR}} &ATOM &\textcolor{red}{(NLP)}  &DW &FC\\
        	           &\textcolor{red}{(NLP)}    &\cite{STARK} &\cite{TrDiMP} & \cite{TransT} &\cite{AutoMatch} & \cite{SiamRCNN} & \cite{Prdimp} &\textcolor{red}{(NLP)}       & \cite{Ocean}   &\cite{SiamCAR} &\cite{Atom} &\cite{SNLT}  &\cite{SiamDW} &\cite{Siamfc}\\
        % 	\midrule
        	\hline
        	
        	AO             & \best{69.4}  & \scnd{68.0} &67.1 & 67.1 &65.2 & 64.9 &63.4 &{61.4}  & 61.1  &56.9  &55.6  &43.3  &42.9  &34.8\\
        	SR$_{0.5}$     & \best{81.1}  & \scnd{77.7} &77.7 & 76.8 &76.6 & 72.8 &73.8 &{72.4}  & 72.1  &67.0  &63.4  &50.6  &48.3  &35.3\\
        	SR$_{0.75}$    & \best{64.5}  & \scnd{62.3} &58.3 & 60.9 &54.3 & 59.7 &54.3 &{52.3}  & 47.3  &41.5  &40.2  &22.1  &14.7  &9.8\\
        	
        % 	\bottomrule
        	\hline
        \end{tabular}
	}
% 	\vspace{-3mm}
	\caption{Comparison on the GOT-10k~\cite{GOT10K} test set ordered by AO. \textit{\textbf{TransT}} and \textit{\textbf{SiamCAR}} are baselines of proposed \textbf{VLT}$_{\mathrm{TT}}$ and \textbf{VLT}$_{\mathrm{SCAR}}$ respectively.
	}
% 	\vspace{-1mm}
	\label{tab:got10k}%
\end{table}

==> tables/lasot.tex <==
\begin{table}[!t]
	\centering
	\vspace{-3mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\opt}[1]{\textbf{\textcolor{violet}{#1}}}
	\newcommand{\fast}[1]{\textbf{\textcolor{orange}{#1}}}
	\newcommand{\dist}{\hspace{3pt}}%
	\renewcommand\arraystretch{1.2}
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}|c@{\dist}|c@{\dist}c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        % 	\toprule
        	\hline
        	           &   & Keep &STARK &   &        & Siam    & Tr  & Pr  &Auto &  &SNLT  &\textit{\textbf{Siam}}  &C-  &\\
        	           & \textbf{VLT}$_{\mathrm{TT}}$  &Track  &st50  & \textbf{VLT}$_{\mathrm{SCAR}}$   & \textit{\textbf{TransT}} & R-CNN  & DiMP  & DiMP &Match &Ocean &\textcolor{red}{(NLP)} &\textit{\textbf{CAR}} &RPN  &PTAV\\
        	           &\textcolor{red}{(NLP)}               & \cite{KeepTrack} &\cite{STARK} & \textcolor{red}{(NLP)} & \cite{TransT} & \cite{SiamRCNN}       & \cite{TrDiMP} & \cite{Prdimp}  &\cite{AutoMatch} &\cite{Ocean} &\cite{SNLT}  &\cite{SiamCAR}  &\cite{C-RPN}  &\cite{PTAV}\\
        % 	\midrule
            \hline
        	
        	Success (AUC)  & \best{67.3}  & \scnd{67.1} & 66.4 &65.2 & 64.9 & 64.8  & 63.9 & 59.8  &58.3 &56.0  &54.0  &50.7  &45.5  &25.0\\
        	Norm. Prec     & \best{78.0}  & \scnd{77.2} & 76.3 &74.9 & 73.8 & 72.2  & 73.0 & 68.8  &62.4 &56.3  &63.6  &60.0  &49.8  &27.4\\
        	Precision      & \best{72.1}  & 70.2 & \scnd{71.2} &69.1 & 69.0 & 68.4  & 66.3 & 60.8  &59.9 &56.6  &57.6  &51.0  &42.5  &24.5\\
        	
        % 	\bottomrule
        	\hline
        \end{tabular}
	}
% 	\vspace{-3mm}
	\caption{Comparison on the LaSOT~\cite{LaSOT} test set ordered by AUC. \textit{\textbf{TransT}} and \textit{\textbf{SiamCAR}} are baselines of proposed \textbf{VLT}$_{\mathrm{TT}}$ and \textbf{VLT}$_{\mathrm{SCAR}}$ respectively.
	}
% 	\vspace{-1mm}
	\label{tab:lasot}%
\end{table}

==> tables/lasot_ext.tex <==
\begin{table}[!t]
	\centering
	\vspace{-3mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\opt}[1]{\textbf{\textcolor{violet}{#1}}}
	\newcommand{\fast}[1]{\textbf{\textcolor{orange}{#1}}}
	\newcommand{\dist}{\hspace{3pt}}%
	\renewcommand\arraystretch{1.3}
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}|c@{\dist}|c@{\dist}c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        % 	\toprule
        	\hline
        	           &   &STARK   &       &   &  &Auto &Siam &\textit{\textbf{Siam}} &C- &SNLT &Siam &Siam & &\\
        	           & \textbf{VLT}$_{\mathrm{TT}}$    &st50     & \textit{\textbf{TransT}} & \textbf{VLT}$_{\mathrm{SCAR}}$ &ATOM &Match &RPN++ &\textit{\textbf{CAR}} &RPN &\textcolor{red}{(NLP)} &DW &FC &ECO &PTAV\\
        	           &\textcolor{red}{(NLP)}              &\cite{STARK} & \cite{TransT} &\textcolor{red}{(NLP)} &\cite{Atom} &\cite{AutoMatch} &\cite{Siamrpn++} &\cite{SiamCAR} &\cite{SNLT} &\cite{C-RPN} &\cite{SiamDW} &\cite{Siamfc} &\cite{ECO} &\cite{PTAV}\\
        % 	\midrule
            \hline
        	
        	Success (AUC)  & \best{48.4}  & \scnd{47.8} & 44.8 &44.7 & 38.8 &37.6  & 35.1 & 33.9  &28.6 &26.2 &24.6  &23.9  &22.7  &20.2\\
        	Norm. Prec     & \best{57.7}  & \scnd{56.2} & 52.3 &53.1 & 46.9 &45.0  & 42.4 & 43.0  &35.2 &31.8 &32.0  &31.8  &25.3  &22.0\\
        	Precision      & \best{55.9}  & \scnd{55.1} & 52.5 &51.6 & 43.5 &43.0  & 40.0 & 41.0  &34.6 &30.0 &25.6  &27.0  &23.7  &22.1\\
        	
        % 	\bottomrule
        	\hline
        \end{tabular}
	}
% 	\vspace{-3mm}
	\caption{Comparison on the LaSOT Extension~\cite{LaSOT_Extention} ordered by AUC. \textit{\textbf{TransT}} and \textit{\textbf{SiamCAR}} are baselines of proposed \textbf{VLT}$_{\mathrm{TT}}$ and \textbf{VLT}$_{\mathrm{SCAR}}$ respectively.
	}
% 	\vspace{-1mm}
	\label{tab:lasot_extention}%
\end{table}

==> tables/otb99.tex <==
\begin{table}[!t]
	\centering
	\vspace{-3mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\opt}[1]{\textbf{\textcolor{violet}{#1}}}
	\newcommand{\fast}[1]{\textbf{\textcolor{orange}{#1}}}
	\newcommand{\dist}{\hspace{3pt}}%
	\renewcommand\arraystretch{1.2}
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}|c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        % 	\toprule
        	\hline
        	           &         &           &Auto  &       &Tr   &Keep &Siam   &STARK &Pr   &\textit{\textbf{Siam}}  &      &     &SNLT &Siam\\
        	           & \textbf{VLT}$_{\mathrm{TT}}$            & \textbf{VLT}$_{\mathrm{SCAR}}$           &Match &\textit{\textbf{TransT}} &DiMP &Track &R-CNN  &st50 &DiMP &\textit{\textbf{CAR}}   &Ocean &ATOM &\textcolor{red}{(NLP)} &FC\\
        	           &\textcolor{red}{(NLP)}  &\textcolor{red}{(NLP)} &\cite{AutoMatch} &\cite{TransT} &\cite{TrDiMP} &\cite{KeepTrack} &\cite{SiamRCNN} &\cite{STARK} &\cite{Prdimp} &\cite{SiamCAR} &\cite{Ocean} &\cite{Atom} &\cite{SNLT} &\cite{Siamfc}\\
        % 	\midrule
        	\hline
        	
        	Success (AUC)  & \best{76.4} &\scnd{73.9} &71.6 &70.8 &70.5 &70.4 &70.0 &69.6 &69.5 &68.8 &68.0 &67.6 &66.6 &58.7\\
        	Norm. Prec     & \best{91.5} &\scnd{88.3} &88.0 &86.1 &86.2 &86.0 &83.7 &85.7 &85.2 &84.9 &85.0 &88.2 &84.8 &74.9\\
        	Precision      & \scnd{93.1} &89.8 &\best{93.2} &91.2 &92.5 &91.5 &89.4 &91.4 &89.5 &89.1 &92.1 &82.4 &80.4 &79.2\\
        	
        % 	\bottomrule
        	\hline
        \end{tabular}
	}
% 	\vspace{-3mm}
	\caption{Comparison on the OTB-99-Lang~\cite{OTB99LANG} test set ordered by AUC. \textit{\textbf{TransT}} and \textit{\textbf{SiamCAR}} are baselines of proposed \textbf{VLT}$_{\mathrm{TT}}$ and \textbf{VLT}$_{\mathrm{SCAR}}$ respectively.
	}
% 	\vspace{-1mm}
	\label{tab:otb99lang}%
\end{table}

==> tables/temp.tex <==
\begin{table}[!t]
% \vspace{-0.5em}
  \caption{Ablation for NAS and NLP on \textbf{VLT}$_{\mathrm{SCAR}}$ and \textbf{VLT}$_{\mathrm{TT}}$.}
  \vspace{-0.5em}
  \label{tab:ablation}
  \begin{center}
  \newcommand{\dist}{\hspace{3pt}}
  \newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
  \newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
  \renewcommand\arraystretch{1.2}
  
  \resizebox{1.00\linewidth}{!}{
  \begin{tabular}{c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}|c@{\dist}c@{\dist}|c@{\dist}c@{\dist}c@{\dist}|c@{\dist}c@{\dist}c@{\dist}|c@{\dist}c@{\dist}c@{\dist}}
  \hline
  \multirow{2}{*}{\#} &\multirow{2}{*}{Method}  &\multicolumn{3}{c|}{Train}  &\multicolumn{2}{c|}{Test} &\multicolumn{3}{c|}{LaSOT} &\multicolumn{3}{c|}{TNL2K} &\multicolumn{3}{c}{GOT-10k} \\
  \cline{8-16}
  & &ASS &ModaMixer &${\mathcal{V}er}_{robust}$ &$\mathcal{L}$ &$\mathcal{L}_{wrong}$ &AUC & P$_{Norm}$ &P &AUC & P$_{Norm}$ &P &AO & SR$_{0.5}$ &SR$_{0.75}$\\
%   \cline{4-6}
  \hline
%   \specialrule{0em}{1pt}{1pt}
  \ding{172}&\textbf{VLT}$_{\mathrm{SCAR}}$ &-       &-        &-	&-	&-  &50.7	&60.0 &51.0 &{35.3} &43.6 &38.4 &56.9 &67.0 &41.5\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{173}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &-        &-	&-	&-  &52.1	&59.8 &50.6 &{40.7} &47.2 &40.2 &54.7 &63.5 &41.2\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{174}&\textbf{VLT}$_{\mathrm{SCAR}}$ &-       &$\surd$  &-  &$\surd$	&-  &57.6	&65.8 &61.1 &{41.5} &49.2 &43.2 &- &- &-\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{175}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &-  &$\surd$	&-	&\best{65.2} &\best{74.9} &\best{69.1} &\scnd{48.3} &\scnd{55.2} &\scnd{46.6} &61.4 &72.4 &52.3\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{176}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &-  &-	&$\surd$	&52.3	&59.2 &54.2 &{38.1} &45.7 &39.6 &50.8 &56.5 &37.4\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{177}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &-  &-	&-  &50.8	&57.9 &52.6 &{39.5} &47.1 &41.2 &52.2 &58.4 &38.7\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{178}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &$\surd$  &$\surd$	&-	&\scnd{63.9} &\scnd{73.3} &\scnd{67.9} &\best{49.8} &\best{58.3} &\best{51.1} &61.0 &70.8 &52.2\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{179}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &$\surd$  &-	&$\surd$	&49.3	&55.6 &51.2 &{38.8} &46.6 &40.5 &51.0 &58.1 &39.2\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{180}&\textbf{VLT}$_{\mathrm{SCAR}}$ &$\surd$ &$\surd$  &$\surd$	&-	&-  &53.4	&60.7 &54.6 &{41.1} &49.1 &42.9 &53.4 &60.4 &40.5\\
  \hline
%   \specialrule{0em}{1pt}{1pt}
  \ding{182}&\textbf{VLT}$_{\mathrm{TT}}$ &-       &-        &-	&-	&-  &64.9	&73.8 &69.0 &{50.7} &57.1 &51.7 &67.1 &76.8 &60.9\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{183}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &-        &-	&-  &-	&63.1	&73.5 &66.5 &{49.3} &55.6 &48.6 & & &\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{184}&\textbf{VLT}$_{\mathrm{TT}}$ &-       &$\surd$  &-  &$\surd$	&-	&-	&- &- & & & & & &\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{185}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &-  &$\surd$	&-	&\scnd{66.3}	&\scnd{77.0} &\scnd{70.5} &\scnd{52.2} &\scnd{58.6} &\scnd{52.1} &68.4 &81.5 &62.4\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{186}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &-  &	&$\surd$	&59.3	&68.6 &62.2 &{49.3} &55.7 &49.2 & & &\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{187}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &-  &-	&-	&60.7	&71.1 &63.1 &{48.2}	&54.6 &46.8 & & &\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{188}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &$\surd$  &$\surd$	&-	      &\best{67.3}	&\best{78.0} &\best{72.1} &\best{53.1} &\best{59.3} &\best{53.3} &69.4 &81.1 &64.5\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{189}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &$\surd$  &-	    &$\surd$  &59.7	&69.2 &63.0 &{50.0} &56.3 &50.3 & & &\\
%   \specialrule{0em}{1pt}{1pt}
  \ding{190}&\textbf{VLT}$_{\mathrm{TT}}$ &$\surd$ &$\surd$  &$\surd$  &-	    &-	      &61.0	&71.5 &63.4 &{49.1} &55.5 &48.3 & & &\\
%   \specialrule{0em}{1pt}{1pt}

  \hline
  \end{tabular}}
  \end{center}
  
  \end{table}

==> tables/tnl2k.tex <==
\begin{table}[!t]
	\centering
	\vspace{-3mm}
	\newcommand{\best}[1]{\textbf{\textcolor{red}{#1}}}
	\newcommand{\scnd}[1]{\textbf{\textcolor{blue}{#1}}}
	\newcommand{\opt}[1]{\textbf{\textcolor{violet}{#1}}}
	\newcommand{\fast}[1]{\textbf{\textcolor{orange}{#1}}}
	\newcommand{\dist}{\hspace{3pt}}%
	\renewcommand\arraystretch{1.2}
	\resizebox{1.00\linewidth}{!}{%
        \begin{tabular}{l@{\dist}|c@{\dist}|c@{\dist}c@{\dist}|c@{\dist}|c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}c@{\dist}}
        % 	\toprule
        \hline
        	           &   &Siam        &   &   & Auto   & Pr  &  &Siam & & &\textit{\textbf{Siam}} &Siam  &Siam &SNLT\\
        	           & \textbf{VLT}$_{\mathrm{TT}}$   &R-CNN  &\textit{\textbf{TransT}}  & \textbf{VLT}$_{\mathrm{SCAR}}$ & Match  & DiMP & KYS  &RPN++ &ATOM &Ocean  &\textit{\textbf{CAR}} &DW &FC &\textcolor{red}{(NLP)}\\
        	           &\textcolor{red}{(NLP)}               & \cite{SiamRCNN}  & \cite{TransT} &\textcolor{red}{(NLP)}       & \cite{AutoMatch} & \cite{Prdimp}  &\cite{Kys}  & \cite{Siamrpn++} &\cite{Atom} &\cite{Ocean} &\cite{SiamCAR} &\cite{SiamDW} &\cite{Siamfc} &\cite{SNLT}\\
        % 	\midrule
        \hline
        	
        	Success (AUC)  & \best{53.1}  & \scnd{52.3} & 50.7 &{49.8}  & 47.2 & 47.0  &44.9  &41.3  &40.1  &38.4  &35.3  &32.3  &29.5  &27.6\\
        	Norm. Prec     & \best{59.3}  & \scnd{57.7} & 57.1 &58.3  & 53.2   & 54.0  &51.1  &48.2  &46.5  &45.4  &43.6  &40.5  &45.0  &35.8\\
        	Precision      & \best{53.3}  & \scnd{52.8} & 51.7 &{51.0}  & 43.5 & 45.9  &43.5  &41.2  &39.2  &37.7  &38.4  &32.6  &28.6  &41.9\\
        	
        % 	\bottomrule
        \hline
        \end{tabular}
	}
% 	\vspace{-3mm}
	\caption{Comparison on the TNL2K~\cite{TNL2K} test set ordered by AUC. \textit{\textbf{TransT}} and \textit{\textbf{SiamCAR}} are baselines of proposed \textbf{VLT}$_{\mathrm{TT}}$ and \textbf{VLT}$_{\mathrm{SCAR}}$ respectively.
	}
% 	\vspace{-1mm}
	\label{tab:tnl2k}%
\end{table}
